An integral equation method for the advection-diffusion equation on time-dependent domains in the plane

Boundary integral methods are attractive for solving homogeneous linear constant coefficient elliptic partial differential equations on complex geometries, since they can offer accurate solutions with a computational cost that is linear or close to linear in the number of discretization points on the boundary of the domain. However, these numerical methods are not straightforward to apply to time-dependent equations, which often arise in science and engineering. We address this problem with an integral equation-based solver for the advection-diffusion equation on moving and deforming geometries in two space dimensions. In this method, an adaptive high-order accurate time-stepping scheme based on semi-implicit spectral deferred correction is applied. One time-step then involves solving a sequence of non-homogeneous modified Helmholtz equations, a method known as elliptic marching. Our solution methodology utilizes several recently developed methods, including special purpose quadrature, a function extension technique and a spectral Ewald method for the modified Helmholtz kernel. Special care is also taken to handle the time-dependent geometries. The numerical method is tested through several numerical examples to demonstrate robustness, flexibility and accuracy

==> results.tex <==
> 1, Lösa modifierade Helmholtz ekvationer med Neumann randdata, i stationär geometri, fri rymd. Det är nytt med:  specialkvadratur för single layer - formuleringen, att ta fram gradienten, Ewald för Yukawa-kärnan. Vi visar konvergensplottar med fel mot upplösning i rummet. Förväntar oss en tionde ordningens metod ned till 1e-10 (gränsen för Ewald pga bibliotek för att beräkna incomplete modified besselfunction).
> 
> 2, Lösa advektion-diffusionekvationen i ett rotationsfält för en stel kropp (deformeras ej). Ingen adaptivitet. Vi visar att vi kan få hög ordning i tiden och att PUX fungerar utmärkt för att fylla i områden där data saknas. Här presenterar vi hela algoritmen och visar att den funkar som den ska. Inkluderar konvergensplottar med fel mot upplösning i tid. Vi presenterar antalet implicita lösningar i förhållande mot felet en viss ordning på SDC gav.
> 
> 3, Lösa advektion-diffusionekvationen i en periodisk kanal. Här introducerar vi periodicitet och ett hastighetsfält som inte är givet analytiskt, samt adaptivitet. Inkluderar konvergensplottar med fel mot upplösning i tid. Även plottar med upplösning i rummet på x-axeln och felet på y-axeln, vill se att olika toleranser uppnås tills upplösningen i rummet är för grov.
> 
> 4, Lösa advektion-diffusionekvationen för en droppe i ett "extensional" flow. Här löser vi Stokes i varje tidssteg (och substeg) och har en deformerbar domän. Här studerar vi endast adaptivitet.
